Real-time Detection and Adaptive Mitigation of Power-based Side-Channel Leakage in SoC

Power-based side-channel is a serious security threat to the System on Chip (SoC). The secret information is leaked from the power profile of the system while a cryptographic algorithm is running. The mitigation requires efforts from both the software level and hardware level. Currently, there is no comprehensive solution that can guarantee the whole complex system is free of leakage and can generically protect all cryptographic algorithms. In this paper, we propose a real-time leakage detection and mitigation system which enables the system to monitor the side-channel leakage effects of the hardware. Our proposed system has extensions that provide a real-time monitor of power consumption, detection of side-channel leakage, and real-time adaptive mitigation of detected side-channel leakage. Our proposed system is generic and can protect any algorithm running on it.

==> biblio_bp.tex <==

@inproceedings{leiserson2014gate,
  title={Gate-level masking under a path-based leakage metric},
  author={Leiserson et al},
  booktitle={International Workshop on Cryptographic Hardware and Embedded Systems},
  pages={580--597},
  year={2014},
  organization={Springer}
}

@inproceedings{wang2019mitigating,
  title={Mitigating power side channels during compilation},
  author={Wang, Jingbo and Sung, Chungha and Wang, Chao},
  booktitle={Proceedings of the 2019 27th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
  pages={590--601},
  year={2019}
}

@inproceedings{gregoire2018vectorizing,
  title={Vectorizing higher-order masking},
  author={Gr{\'e}goire, Benjamin and Papagiannopoulos, Kostas and Schwabe, Peter and Stoffelen, Ko},
  booktitle={International Workshop on Constructive Side-Channel Analysis and Secure Design},
  pages={23--43},
  year={2018},
  organization={Springer}
}

@article{gao2020share,
  title={Share-slicing: Friend or Foe?},
  author={Gao, Si and Marshall, Ben and Page, Dan and Oswald, Elisabeth},
  journal={IACR Transactions on Cryptographic Hardware and Embedded Systems},
  pages={152--174},
  year={2020}
}

@inproceedings{kocher2019spectre,
  title={Spectre attacks: Exploiting speculative execution},
  author={Kocher, Paul and Horn, Jann and Fogh, Anders and Genkin, Daniel and Gruss, Daniel and Haas, Werner and Hamburg, Mike and Lipp, Moritz and Mangard, Stefan and Prescher, Thomas and others},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={1--19},
  year={2019},
  organization={IEEE}
}

@article{depoix2018detecting,
  title={Detecting Spectre Attacks by identifying Cache Side-Channel Attacks using Machine Learning},
  author={Depoix, Jonas and Altmeyer, Philipp},
  journal={Advanced Microkernel Operating Systems},
  volume={75},
  year={2018}
}

@inproceedings{homma2014attack,
  title={Em attack is non-invasive?-design methodology and validity verification of em attack sensor},
  author={Homma, Naofumi and Hayashi, Yu-ichi and Miura, Noriyuki and Fujimoto, Daisuke and Tanaka, Daichi and Nagata, Makoto and Aoki, Takafumi},
  booktitle={International Workshop on Cryptographic Hardware and Embedded Systems},
  pages={1--16},
  year={2014},
  organization={Springer}
}

@article{utyamishev2018real,
  title={Real-Time Detection of Power Analysis Attacks by Machine Learning of Power Supply Variations On-Chip},
  author={Utyamishev, Dmitry and Partin-Vaisband, Inna},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={1},
  pages={45--55},
  year={2018},
  publisher={IEEE}
}

@inproceedings{becker2013test,
  title={Test vector leakage assessment (TVLA) methodology in practice},
  author={Becker, George and Cooper, J and DeMulder, Elke and Goodwill, Gilbert and Jaffe, Joshua and Kenworthy, G and Kouzminov, T and Leiserson, A and Marson, M and Rohatgi, Pankaj and others},
  booktitle={International Cryptographic Module Conference},
  volume={1001},
  pages={13},
  year={2013}
}

@inproceedings{de2019protecting,
  title={Protecting RISC-V against Side-Channel Attacks},
  author={De Mulder, Elke and Gummalla, Samatha and Hutter, Michael},
  booktitle={2019 56th ACM/IEEE Design Automation Conference (DAC)},
  pages={1--4},
  year={2019},
  organization={IEEE}
}

@inproceedings{barthe2017parallel,
  title={Parallel implementations of masking schemes and the bounded moment leakage model},
  author={Barthe, Gilles and Dupressoir, Fran{\c{c}}ois and Faust, Sebastian and Gr{\'e}goire, Benjamin and Standaert, Fran{\c{c}}ois-Xavier and Strub, Pierre-Yves},
  booktitle={Annual International Conference on the Theory and Applications of Cryptographic Techniques},
  pages={535--566},
  year={2017},
  organization={Springer}
}

@inproceedings{wu2018eliminating,
  title={Eliminating timing side-channel leaks using program repair},
  author={Wu, Meng and Guo, Shengjian and Schaumont, Patrick and Wang, Chao},
  booktitle={Proceedings of the 27th ACM SIGSOFT International Symposium on Software Testing and Analysis},
  pages={15--26},
  year={2018}
}


@inproceedings{goudarzi2018secure,
  title={Secure multiplication for bitslice higher-order masking: Optimisation and comparison},
  author={Goudarzi, Dahmun and Journault, Anthony and Rivain, Matthieu and Standaert, Fran{\c{c}}ois-Xavier},
  booktitle={International Workshop on Constructive Side-Channel Analysis and Secure Design},
  pages={3--22},
  year={2018},
  organization={Springer}
}

@inproceedings{brier2004correlation,
  title={Correlation power analysis with a leakage model},
  author={Brier, Eric and Clavier, Christophe and Olivier, Francis},
  booktitle={International workshop on cryptographic hardware and embedded systems},
  pages={16--29},
  year={2004},
  organization={Springer}
}

@inproceedings{kocher1999differential,
  title={Differential power analysis},
  author={Kocher, Paul and Jaffe, Joshua and Jun, Benjamin},
  booktitle={Annual International Cryptology Conference},
  pages={388--397},
  year={1999},
  organization={Springer}
}

@inproceedings{zhao2018fpga,
  title={FPGA-based remote power side-channel attacks},
  author={Zhao, Mark and Suh, G Edward},
  booktitle={2018 IEEE Symposium on Security and Privacy (SP)},
  pages={229--244},
  year={2018},
  organization={IEEE}
}

@article{moradi2018leakage,
  title={Leakage detection with the x2-test},
  author={Moradi, Amir and Richter, Bastian and Schneider, Tobias and Standaert, Fran{\c{c}}ois-Xavier},
  journal={IACR Transactions on Cryptographic Hardware and Embedded Systems},
  pages={209--237},
  year={2018}
}

@article{bronchain2019multi,
  title={Multi-Tuple Leakage Detection and the Dependent Signal Issue},
  author={Bronchain, Olivier and Schneider, Tobias and Standaert, Fran{\c{c}}ois-Xavier},
  journal={IACR Transactions on Cryptographic Hardware and Embedded Systems},
  pages={318--345},
  year={2019}
}

@inproceedings{ishai2003private,
  title={Private circuits: Securing hardware against probing attacks},
  author={Ishai, Yuval and Sahai, Amit and Wagner, David},
  booktitle={Annual International Cryptology Conference},
  pages={463--481},
  year={2003},
  organization={Springer}
}

@inproceedings{balasch2014cost,
  title={On the cost of lazy engineering for masked software implementations},
  author={Balasch, Josep and Gierlichs, Benedikt and Grosso, Vincent and Reparaz, Oscar and Standaert, Fran{\c{c}}ois-Xavier},
  booktitle={International Conference on Smart Card Research and Advanced Applications},
  pages={64--81},
  year={2014},
  organization={Springer}
}

@inproceedings{papagiannopoulos2017mind,
  title={Mind the gap: towards secure 1st-order masking in software},
  author={Papagiannopoulos, Kostas and Veshchikov, Nikita},
  booktitle={International Workshop on Constructive Side-Channel Analysis and Secure Design},
  pages={282--297},
  year={2017},
  organization={Springer}
}

@article{kiaei2020domain,
  title={Domain-Oriented Masked Instruction Set Architecture for RISC-V.},
  author={Kiaei, Pantea and Schaumont, Patrick},
  journal={IACR Cryptol. ePrint Arch.},
  volume={2020},
  pages={465},
  year={2020}
}
